A Novel Graphical Lasso based approach towards Segmentation Analysis in Energy Game-Theoretic Frameworks

Energy game-theoretic frameworks have emerged to be a successful strategy to encourage energy efficient behavior in large scale by leveraging human-in-the-loop strategy. A number of such frameworks have been introduced over the years which formulate the energy saving process as a competitive game with appropriate incentives for energy efficient players. However, prior works involve an incentive design mechanism which is dependent on knowledge of utility functions for all the players in the game, which is hard to compute especially when the number of players is high, common in energy game-theoretic frameworks. Our research proposes that the utilities of players in such a framework can be grouped together to a relatively small number of clusters, and the clusters can then be targeted with tailored incentives. The key to above segmentation analysis is to learn the features leading to human decision making towards energy usage in competitive environments. We propose a novel graphical lasso based approach to perform such segmentation, by studying the feature correlations in a real-world energy social game dataset. To further improve the explainability of the model, we perform causality study using grangers causality. Proposed segmentation analysis results in characteristic clusters demonstrating different energy usage behaviors. We also present avenues to implement intelligent incentive design using proposed segmentation method.

==> socialGame.tex <==
\section{Gamification in Human Centric Cyber-Physical Systems}\label{game_desc}

\begin{figure}[!ht]
\centering
  \includegraphics[width=0.45\textwidth]{figs/gamification_abstraction5}
  \caption{Gamification abstraction for \textit{Human Centric Cyber-Physical Systems} towards building energy efficiency}
  \label{fig:gamification_abstraction}
\end{figure}

We envision smart-building systems in which humans take control, interact, and improve the environment they inhabit. Figure ~\ref{fig:gamification_abstraction} shows a generalized gamification abstraction towards enabling strategic interactions among non-cooperative agents in \textit{Human-Centric Cyber-Physical Systems}. The broader purpose of this section is to present a general gamification framework that leverages game-theoretic concepts to learn models of player's decision making in competitive environments such as a smart building.

\subsection{Game theoretic framework}\label{game_model}

In this section, we abstract the agent's decision making process in a game-theoretic framework using discrete choice theory~\cite{train2009discrete}. Under a discrete choice model, the decision of an agent can be predicted from a given choice set using a variety of available features. For our case, the features are dorm-room energy resource (desk light, ceiling light, ceiling fan) usage.

\subsubsection{Agent decision-making model}

Consider an agent $i$ and the decision-making choice set indexed by the set $\mc{I}=\{\mc{J}^1,\ldots, \mc{J}^S \}$. A player $i$ chooses between $S$ alternative choices and would earn a \textbf{representative utility} $f_i$ for $i \in \mc{I}$. Each decision by the players leads them to get the highest possible utility, $f_i > f_j$ for all $i,j \in \mc{I}$. In our formulation, an agent has a utility which depends on a number of features $x_z$ for $z=1, \ldots, N$. However, there are several unobserved features of the representative utility which are treated as random variables. Hence, the \textbf{random utility} decision-making model for each player is given by 

\begin{equation}
  \hat{f}_i(x)=g_i(\beta_{i},x) + \epsilon_{i}
  \label{eq:discrete_utility}
\end{equation}

where $\epsilon_{i}$ is the unobserved random component of the agent's utility and $g_i(\beta_{i},x)$ is a nonlinear generalization of agent $i$'s utility function where

\begin{equation}
x=(x_1, \ldots, x_{i-1}, x_{i+1}, \ldots, x_N)\in \mb{R}^{N} 
\label{eq:feature}
\end{equation} 

is the collective $n$ features explaining an agent's decision process. The choice of nonlinear mapping $g_i$ and $x$ abstracts the agent's decision. This is an adaptation of their classical representation~\cite{train2009discrete} using a linear mapping $g_i(\beta_{i},x) = \beta_{i}^{T}x$ in which $\epsilon_{i}$ is an independently and identically distributed random value modeled using a Gumbel distribution. In general, each player is modeled as a \emph{utility maximizer} that seeks to select $i\in \mc{I}$ by optimizing \eqref{eq:discrete_utility}.

% is the
% collective $n$ features explaining an agent's decision process. The choice of nonlinear mapping $g_i$ and $x$ abstracts the agent's decision; it could represent, e.g.,
% how much of a particular resource they choose to use and when an agent optimizes its usage over a specific resource. This is an adaptation of their classical

\subsubsection{Game formulation}

We use a \emph{sequential non-cooperative discrete game} concept to model the outcome of the strategic interactions between players. The random utility in a generalized decision-making model for each agent~\eqref{eq:discrete_utility} can be modeled either with linear or nonlinear mapping, a sequential non-cooperative discrete game is given by:

%\begin{definition}

Each agent $i$ has a set $\mc{F}_i = {f_{i}^1,\ldots, f_{i}^{N}}$ of $N$ \textbf{random utilities}. Each random utility $j$ has a convex decision-making choice set $\mc{I}_{j}=\{\mc{J}^{1}_{j},\ldots, \mc{J}^{S}_{j} \}$. Given a collection of $n$ features~\eqref{eq:feature} comprising the decision process, where the temporal parameter $T$ is also given, agent $i$ faces the following optimization problem for its \textbf{aggregated random utility}:

\begin{equation}
  \max\{\sum_{i=1}^{N}f^{T}_i(x)|\  f_i \in \mc{F}_i\}.
  \label{eq:opt-seq}
\end{equation}
%\end{definition}

In the sequential equilibrium concept, agents in the game independently co-optimize their aggregated random utilities~\eqref{eq:opt-seq} given a collective of $n$ features~\eqref{eq:feature} at each time instance $T$ (temporal parameter).


\subsection{Human-centric CPS experiment}\label{social_game}

% \begin{figure}[!ht]
% \includegraphics[width=0.45\textwidth,center]{pics/game_utilization.pdf}
% \caption{Graphical user interface (GUI)}
% \label{fig:game_utilization_design}
% \end{figure}

\iffalse
\begin{figure*}[!ht]
\center    \subfigure[\label{fig:game_utilization}]{\includegraphics[width=0.38\textwidth]{figs/game_utilization.pdf}}
    \subfigure[\label{fig:IoT_design}]{\includegraphics[width=0.407\textwidth]{figs/IoT_design.pdf}}
  \caption{Graphical user interface (GUI) and dataflow design for energy-based social game}
  \label{fig:game_utilization_design}
\end{figure*}
\fi

% \begin{figure}[!ht]
%     \subfloat[Graphical user interface (GUI) for energy-based social game: Display of consumption for resources, real-time feedback for device status (on/off), daily counter, and random coin]{%
%     \includegraphics[width=0.25\textwidth]{pics/game_utilization.pdf}
%     }
%     \hfill
%     \subfloat[Social game dataflow architecture design]{%
%     \includegraphics[width=0.25\textwidth]{pics/IoT_design.pdf}
%     }
% \caption{Graphical user interface (GUI) and dataflow design for energy-based social game}
% \label{fig:game_utilization_design}
% \end{figure}

Using the \emph{Game theoretic framework} presented in section \ref{game_model}, we designed a social game experiment encourage energy efficient resource consumption in a smart residential housing which included residential housing single room apartments at Nanyang Technological University (NTU) campus. We refer interested readers to this paper~\cite{konstantakopoulos2018deep}, which includes the details of the experiment\footnote{For demonstrations of our infrastructure and for downloading de-identified high dimensional data, please visit our web site: \href{url}{https://smartntu.eecs.berkeley.edu}}. 
\iffalse
Monitoring past energy usage data for approximately one month before the introduction of the game for each semester, we calculated the baselines for each of the occupant's resources. Using this prior data, a weekday and weekend baseline was assigned. We accumulated data separately for weekdays and weekends so as to maintain fairness for occupants who have alternative schedules of occupancy (e.g. those who tend to stay at their dorm room over the weekends versus weekdays). Then, after introduction of the social game, dorm occupants were rewarded with points based on how energy efficient their daily usage is in comparison to their baseline usage.  We employed a lottery mechanism consisting of gifts awarded on a bi-weekly basis to incentivize occupants; occupants with more points are more likely to win the lottery. Earned points for each resource is given by

\begin{equation}
  \hat{p}^{d}_{i}(b_i, u_{i})= s_{i} \frac{b_i - u^{d}_{i}}{b_i}
  \label{eq:points_earned}
\end{equation}

where $\hat{p}^{d}_{i}$ is the points earned at day $d$ for room's resource $i$ which corresponds to ceiling light, desk light, ceiling fan, and A/C. Also, $b_i$ is the baseline calculated for each resource $i$, $u^{d}_{i}$ is the usage of the resource at day $d$, and $s_{i}$ is a points booster for inflating the points as a process of framing \cite{tversky1981framing}.

In Figure~\ref{fig:game_utilization_design}, we present how our graphical user interface was capable of reporting to occupants the real-time status (on/off) of their devices, their accumulated daily usage, time left for achieving daily baseline, and the percentage of allowed baseline being used by hovering above their utilization bars. In order to boost participation, we introduced a randomly appearing coin close to the utilization bars with the purpose of incentivizing occupants to log in to web-portal and view their usage. The residential housing single room apartments on the Nanyang Technological University campus were divided into four blocks, each of which had two levels. In this space, there were a total of seventy-two occupants who were eligible to participate in the social game. Participation in our social game platform was voluntary. We ran the experiment in both the Fall 2017 (September 12th - December 3rd) and Spring 2018 (February 19th - May 6th) semesters.
We enabled the design and implementation of a large-scale networked social game through the utilization of cutting-edge Internet of Things (IoT) sensors, advanced computational hardware devices (Raspberry Pi) and local weather monitoring station---systems (as an external parameter for our model). The actual data-feed was implemented through enabled 4G Wi-Fi Network in Singapore followed by posting of data(with minimal latency) to OSIsoft PI database \footnote{\textit{OSIsoft PI database}: https://www.osisoft.com} located at the University of California, Berkeley campus. The actual design and dataflow is depicted in Figure~\ref{fig:game_utilization_design}. 

Leveraging several indoor metrics like indoor illuminance, humidity, temperature, and vibrations (ceiling fan sensor), we derived simple thresholds indicating if a resource is in use or not. For instance, the standard deviation of acceleration derived from the ceiling fan mounted sensor is an easy way to determine whether ceiling fan is in the on state. Our calibrated detection thresholds are robust over daylight patterns, external humidity/temperature patterns, and noisy measurements naturally acquired from IoT sensors. While we were getting streamed data from various sensors in all dorm rooms, our back-end processes updated the status of the devices in near real-time in each occupant's account and updated points based on their usage and points calculation formula \eqref{eq:points_earned}. This functionality allowed occupants to receive feedback for their actions and view their points balance and their ranking among other capabilities.
\fi
% \begin{figure}[!ht]
% \includegraphics[width=0.45\textwidth,center]{pics/ceiling_fan_status.png}
% \caption{Patterns for ceiling fan resource at a dorm room. The on pulses point to instances that the thresholding system indicates activity in the device.}
% \label{fig:device_status}
% \end{figure}
\subsection{Social game data set}\label{social_game_data_set}

We aggregated occupant's data from the experiment in per-minute resolution. The features include time-stamp, each resource's status, accumulated resource usage (in minutes) per day, resource baseline, gathered points (both from game and surveys), occupant rank in the game over time and occupant's number of visits to the game web portal. In addition to these features, we add several external weather metrics like humidity, temperature, and solar radiation among others. We pool more features by leveraging domain knowledge and external information. Specifically, we consider \textbf{college schedule dummy feature indicators} including periods related to breaks, holidays, midterm and final exam periods at NTU to capture occupant's variability in normal usage of their dorm room resources. Moreover, we include \textbf{seasonal dummy feature indicators} like time of day (morning vs. evening) and time of week (weekday vs. weekend) to capture occupant's seasonal patterns in resource usage.

  
% \begin{enumerate}
%     \item \textbf{College schedule dummy feature indicators:} including dummy variables for dates related to breaks, holidays, midterm period, and the final exam schedule at Nanyang Technological University. These features can capture occupants' variability of normal usage of their dorm room resources.
%     \item \textbf{Seasonal dummy feature indicators:} we compute several seasonal dummy variables utilizing our time-stamps. Examples of seasonal variables are time of day (morning vs. evening) and time of week (weekday vs. weekend) indicators. The intuition behind such features is their ability to capture occupants' seasonal patterns in resource usage. 
%     \item \textbf{Resources status continuous features:} we incorporate stream resource status data for defining pooled features that accurately model occupants variability in resources usage across each day. Examples of such pooled features are: frequency of resource daily switches and percentage of resource usage across the day. 
% \end{enumerate}
